Contextual Documentation Referencing on Stack Overflow

Software engineering is knowledge-intensive and requires software developers to continually search for knowledge, often on community question answering platforms such as Stack Overflow. Such information sharing platforms do not exist in isolation, and part of the evidence that they exist in a broader software documentation ecosystem is the common presence of hyperlinks to other documentation resources found in forum posts. With the goal of helping to improve the information diffusion between Stack Overflow and other documentation resources, we conducted a study to answer the question of how and why documentation is referenced in Stack Overflow threads. We sampled and classified 759 links from two different domains, regular expressions and Android development, to qualitatively and quantitatively analyze the links' context and purpose, including attribution, awareness, and recommendations. We found that links on Stack Overflow serve a wide range of distinct purposes, ranging from citation links attributing content copied into Stack Overflow, over links clarifying concepts using Wikipedia pages, to recommendations of software components and resources for background reading. This purpose spectrum has major corollaries, including our observation that links to documentation resources are a reflection of the information needs typical to a technology domain. We contribute a framework and method to analyze the context and purpose of Stack Overflow links, a public dataset of annotated links, and a description of five major observations about linking practices on Stack Overflow. We further point to potential tool support to enhance the information diffusion between Stack Overflow and other documentation resources.

==> s9-relwork.tex <==
\section{Related Work}
\label{s:relwork}

%\todo{extend and revise this section}
%\todo{move upwards to help motivating what our study adds to the body of knowledge?}

% There have been different studies investigating individual aspects of link usage on Stack Overflow. Gomez et al.~\cite{GCS2013a} conducted a preliminary study of the links found on Stack Overflow. % performed in the context of the MSR 2013 Challenge.
% However, their study focused on the different types of links in posts (not comments) and it did not factor in a distinction based on the domain. In this paper, we investigate two specific domains, which allows us to understand the data in a specific context. Moreover, we integrate an analysis of the purpose of the information sharing that goes beyond a basic description of its nature.
%
% Vincent et al.~\cite{VJH2018a} analyzed the usage of Wikipedia by Stack Overflow authors. Their work is closely related to the purpose \textsc{Concept} in our coding schema. Although we found this purpose to be associated with Wikipedia links, our notion of \textsc{Concept} is not limited to this particular website. Vincent et al. found that 1.28\% of all Stack Overflow posts contain links to Wikipedia. Using version 2018-07-31 of the \emph{SOTorrent}~dataset~\cite{BDTD2018}, we identified 1.94\% of all threads, but only 0.85\% of all posts, to contain links to Wikipedia.
% Also considering links in comments, which Vincent et al. did not, the ratio of threads with links to Wikipedia increases to 2.55\%.
% %\todo{SB: I'm pretty sure that Vincent et al. mixed up x \% of all posts with x \% of all threads. Is this paragraph too offensive towards Vincent et al.?}

% Li et al.~\cite{LXS2018} built a collaborative filtering recommender system to recommend other learning resources, which is based on co-occurrences of links in Stack Overflow posts.
%A piece of work to discuss in our motivation and implication section. Same idea with \cite{LXK2018a, LSX2018a, LXY2016a}.
%\textbf{Srba and M. Bielikova SW 2016}\cite{SB2016a} argue, with stats, that SO might be failing. Something to cite as motivation in the intro?
%\textbf{Rosen and Shihab ESE 2016}\cite{RS2016a} have topic modeling study of mobile development questions, which we could use as context.
% As outlined above, the purpose-resource correspondence that we identified may help to improve such recommender systems.

% REMOVED Xia et al.~\cite{XiaBaoOthers2017} describe that it is common for developers to search for reusable code snippets on the web.
% In particular when developers want to copy such snippets into their projects, \textsc{Attribution} links can be helpful to decide under which license the content can be used, a problem which many developers are not aware of~\cite{SD2018}.

% Treude and Robillard~\cite{TreudeRobillard2017} conducted a survey to investigate whether Stack Overflow code fragments are self-explanatory and found that less than half of the fragments in their sample were considered to be self-explanatory.
% Providing links to related documentation resources may help developers in understanding such code fragments.
%\textbf{Nasehi et al.}\cite{NasehiSillitoOthers2012} describe characteristics of effective code examples.

% To describe topics of Stack Overflow questions and answers, different methods such as manual analysis~\cite{TreudeBarzilayOthers2011} and Latent Dirichlet Allocation~\cite{WangLoDavidOthers2013, AllamanisSutton2015} have been used.
% Automatically identifying high-quality posts has been another research direction, where metrics based on the number of edits on a question~\cite{YangHauffOthers2014}, author popularity~\cite{PonzanelliMocciOthers2014}, and code readability~\cite{DuijnKuceraOthers2015} yielded good results.
% To identify the topics and assess the quality of Stack Overflow posts, linked documentation resources, and in particular their correspondence to certain link purposes, could be used in future work.
%
% In their conceptual framework of success factors for Stack Overflow questions, Calefato et al.~\cite{CalefatoLanubileOthers2018} considered the presence of links as one aspect of a question's presentation quality.
% However, they did not find a significant effect of the fact that a question contained a link on the the success of that question, that is whether it attracted an accepted answer.
% A direction of future work is to consider not only the presence of a links, but also their purpose and targets.

% Outside of Stack Overflow, Hata et al.~\cite{Hata2019} studied the role of links contained in source code comments in terms of prevalence, link targets, purposes, decay, and evolutionary aspects. Similar to our findings, Hata et al.~also report that link can be fragile since they are vulnerable to link rot and link targets change frequently.

